CC-Cert: A Probabilistic Approach to Certify General Robustness of Neural Networks

In safety-critical machine learning applications, it is crucial to defend models against adversarial attacks -- small modifications of the input that change the predictions. Besides rigorously studied $\ell_p$-bounded additive perturbations, recently proposed semantic perturbations (e.g. rotation, translation) raise a serious concern on deploying ML systems in real-world. Therefore, it is important to provide provable guarantees for deep learning models against semantically meaningful input transformations. In this paper, we propose a new universal probabilistic certification approach based on Chernoff-Cramer bounds that can be used in general attack settings. We estimate the probability of a model to fail if the attack is sampled from a certain distribution. Our theoretical findings are supported by experimental results on different datasets.

==> contents/0.abstract.tex <==
Robustness and certification are totally important:)

\todo{1. plan the paper}

==> contents/extradata.tex <==
\paragraph{Confidence interval for the mean.}
It has been observed earlier\footnote{ZHOU, X.-H., \& GAO, S. (1997). CONFIDENCE INTERVALS FOR THE LOG-NORMAL MEAN. Statistics in Medicine, 16(7)}, that the confidence interval for lognormal  random variables (rvs) has the following form:
\begin{equation}
    \hat y = \frac1n\sum_i\exp(X_i),\quad  X_i\sim\mathcal N(\mu,\,\sigma),
    \label{eq:lognormalmean}
\end{equation}
with unknown $\mu$ and $\sigma$.
The following upperbound is considered:
$$
\theta^{\text{up}} = \hat\mu + \hat\sigma^2/2 + \frac q{\sqrt n}\sqrt{\hat\sigma^2(1+\hat\sigma^2/2)},
$$
where $\hat\mu$ is sample mean and $\hat\sigma^2$ is unbiased sample variance if $X_i$ rvs, i.e.
$$
\hat\mu=\frac1n\sum_{i=1}^nX_i,\quad
\hat\sigma^2=\frac1{n-1}\sum_{i=1}^n(X_i-\hat\mu)^2.
$$
The value of~$q$ depends on the desired quantile and is usually set to $q\approx2$. (An analogous formalu exists for the lower bound as well). Having the expression for $\theta^{\text{up}}$, we can derive the upper bound formula for the random variable in~\eqref{eq:lognormalmean}
$$
y^{\text{up}}=\exp\theta^{\text{up}}.
$$
And finally we can write out the upper bounds expression for the inital rv in ~\eqref{eq:main} as a function of~$t$,
\begin{equation}
Y^{\text{up}}=\exp\left\{
    t\hat\mu  + t^2\hat\sigma^2/2  + t\frac q{\sqrt n}\sqrt{\hat\sigma^2(1+t^2\hat\sigma^2/2)}
-at
    \right\}.
    \label{eq:yup}
\end{equation}
$Y^{\text{up}}$ has the only global minimum over $t$ for $t\in[0,\,\infty]$, which immediately yields the upper bounds value itself for rv $Y$.
Despite the normal distribution of the rvs $X_i$ in~\eqref{eq:lognormalmean}, in what follows we show numerically that the upper bound works well for uniform distribution.

\paragraph{Numerical experiments.}
The table below shows the calculated upper bound $Y^{\text{up}}$ of the confidence interval of rv in~\eqref{eq:main} over different values of the number of samples $n$ and parameter~$a$.
For some cofigurations of the parameters, we plot the function $Y^{\text{up}}$ in the figures below.
\begin{table}[]
    \centering
    \begin{tabular}[h]{c||c|c|c||c}
        $X_i$ & $n$ & $a$ & $t_{\text{min}} $ & $Y^{\text{up}}(t_{\text{min}})$ \\\hline
$\mathcal U(0,\,1)$ & 100 & 1 & 4.26154 & 0.387197\\\hline
$\mathcal U(0,\,1)$ & 1000 & 1 & 5.42482 & 0.268035\\\hline
$\mathcal U(0,\,1) $ & 100 & 1.2 & 6.27384 & 0.117551\\\hline
$\mathcal U(0,\,1)$ & 1000 & 1.2 & 8.04348 & 0.0622941\\\hline
$\mathcal U(0,\,1)$ & 100 & 1.5 & 9.33083 & 0.0111136\\\hline
$\mathcal U(0,\,1)$ & 1000 & 1.5 & 11.1443 & 0.00414658\\\hline

$\mathcal N(0,\,1)$ & 1000 & 1 & 0.928165 & 0.642223\\\hline
$\mathcal N(0,\,1)$ & 100 & 1.5 & 1.10077 & 0.505314\\\hline
$\mathcal N(0,\,1)$ & 1000 & 1.5 & 1.16611 & 0.428194\\\hline
$\mathcal N(0,\,1)$ & 100 & 3 & 2.3261 & 0.0307293\\\hline
$\mathcal N(0,\,1)$ & 1000 & 3 & 2.64167 & 0.0187832\\\hline
$\mathcal N(0,\,3)$ & 100 & 3 & 0.245549 & 0.756383\\\hline
$\mathcal N(0,\,3)$ & 1000 & 3 & 0.266487 & 0.685306\\\hline
$\mathcal N(0,\,3)$ & 100 & 9 & 0.680637 & 0.0587438\\\hline
$\mathcal N(0,\,3)$ & 1000 & 9 & 0.97158 & 0.0129443\\\hline
    \end{tabular}
    \caption{Upper bound $Y^{\text{up}}$ over some instantiations of $X_i$ distribution, number of samples $n$, and parameter $a$} 
\end{table}

\def\gr#1#2#3#4{
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/#1_#2,a=#3,ms=#4.pdf}
    \caption{Upper bound $Y^{\text{up}}$ dependency on $t$}
    \label{fig:Y_#1_#2,a=#3,ms=#4}
\end{figure}
\par
}


\gr N{100}93
\gr N{1000}31
\gr N{1000}11
\gr U{1000}{1.5}1
\gr U{1000}11
\FloatBarrier

\paragraph{Analytical derivation.}
We aim to find a distribution $F_n$ of the random variable 
$$
\frac1n\sum_{i=1}^n\exp(X_it).
$$

The density of the rv $\exp(t X)$ is
\begin{equation}
f(y)=
\frac{\theta (y-1) \theta \left(e^t-y\right)}{t y},
\label{eq:rho}
\end{equation}
where $\theta$ is a Heaviside function.

Useful properties of $\exp(t X)$:
\begin{itemize}
    \item mean 
        \begin{equation}
            \displaystyle\mu=\frac{e^t-1}{t}
            \label{eq:mu}
        \end{equation}
    \item variance 
        \begin{equation}
            \displaystyle\sigma^2=\frac{e^t t \sinh (t)-\left(e^t-1\right)^2}{t^2}
            \label{eq:sigma}
        \end{equation}

    \item third moment \newline
    $\rho=\mathbb E\left((X-\mu)^3\right)=\displaystyle
\frac{2 e^{3 t/2} \sinh
   \left(\frac{t}{2}\right) \left(t^2+2 \left(t^2+6\right) \cosh (t)-9 t \sinh (t)-12\right)}{3
   t^3}$
\end{itemize}

We can now estimate the cumulative function $F_n$ with the help of Berry–Esseen theorem, which states that, under certain circumstances, the probability distribution of the scaled mean of a random sample converges to a normal distribution as the sample size increases to infinity. In particular, the Berry-Esseen inequality gives us a bound on the approximation error:
\begin{equation}
    \left|F_n(x)-\mathcal N\bigl(x|\mu,\,\sigma/\sqrt n \bigr)\right| \leq \frac{C \rho}{\sigma^4n},
    \label{eq:BE}
\end{equation}
where $C$ has an estimate $C<0{,}4784$. Because the right hand side of the expression has a fast growth with~$t$ (see Figure~\ref{fig:rhs}), we should either take smaller $t$ values or large number of samples $n$.

\begin{figure}[h!]
    \centering
\includegraphics[width=0.6\linewidth]{figures/BerryEsseen.pdf}
    \caption{The right hand side in the Berry-Esseen estimate.}
    \label{fig:rhs}
\end{figure}

\paragraph{Numerical estimate.} We can roughly estimate the density via convolving the discrete probabilities vector with itself $n$ times. We can compute this convolution  with the Fast Fourier Transform (FFT).

Let us fix the frequency of dicretization~$m$ and form a vector $\{v_i\}_{i=1,..,m}$
$$
v_i=\frac1t\Biggl(
    \log\left(1+\frac{e^t-1}mi\right)-
    \log\left(1+\frac{e^t-1}m(i-1)\right)
\Biggr),
$$
which has a physical meaning of a probability of the $e^{tX}$ rv being in every of the $m$ equal intervals of the range $[1,\,e^t]$.
We then add $(n-1)(m-1)$ zeros to this vector (on the right end), we denote this vector $V$.

The desired probabilities $W=\{w_i\}_{i=1,\dots,n(m-1)+1}$ are obtained by applying FFT, element-wise power operation and applying inverse Fourier transform
$$
W=\mathcal F^{-1}[  \mathcal F[V] ^n  ].
$$
We show the resulting probabilities (points) and limiting density of the normal distribution (lines) on the Figure~\ref{fig:empirical}. Here we set $m=20$, $n=5$. Even with the small $n$ we can see a good convergence.
\begin{figure}[h!]
    \centering
\includegraphics[width=0.9\linewidth]{figures/all-Ch-K.pdf}
    \caption{Empirical densities of the distribution with different $t$.}
    \label{fig:empirical}
\end{figure}

The following can also reveal an approximation error of the discretized approach. We should take the probability values with surplus and shortage
$$
v_i^{\text{min}}=\frac1t\Biggl(
    \log\left(1+\frac{e^t-1}m(i-1/2)\right)-
    \log\left(1+\frac{e^t-1}m(i-3/2)\right)
\Biggr),
$$
$$
v_i^{\text{max}}=\frac1t\Biggl(
    \log\left(1+\frac{e^t-1}m(i+1/2)\right)-
    \log\left(1+\frac{e^t-1}m(i-1/2)\right)
\Biggr),
$$
then the probabilities (only nominally, they do niot sum to 1)
$W^{\text{min}}$ and
$W^{\text{max}}$ will bound the unknown probability. We accounted for the monotonicity of
$
\log\left(1+\frac{e^t-1}mi\right)
$ as a function of~$i$.

We can now numerically estimate the approximation error. A relative error is bounded
$$
\frac{v_i^{\text{max}}-
v_i^{\text{min}}}{v_i}
\leq
\frac{e^t-1}m%\frac{e^t-1}{tm}
$$

Since each component of $\mathcal F[V]$ (after applying FFT) is obtained by multiplying a matrix with unit elements in absolute value, we can roughly estimate the relative error after power operation as follows.
$$
 \left|   \frac{(\mathcal F[V^{\text{min}}]^n)_j-
    (\mathcal F[V^{\text{max}}]^n)_j}
    {(\mathcal F[V]^n)_j}
\right|
    \leq
    %\frac{\frac{(e^t-1)^2}{mt}n}{df}
    %,\quad \forall j.
    \frac{e^t-1}mn.
$$
%Далее, при получении окончательного вектора, снова умножаем матрицу с единичными элементами на этот вектор,
%и с учётом нормировочного множителя $\sim 1/(mn)$, входящего в определение обратного преобразования Фурье, получаем
We expect that the final relative error will also be the same
$$
\left|
\frac{W^{\text{max}}- W^{\text{min}}}W
\right|\leq
%\left(\frac{(e^t-1)^2}{mt}\right)^n.
\frac{e^t-1}mn.
$$
We mention again, that the estimate is quite roughly derived. However, it allows for a rough estimate of the dscretization steps~$m$.

There are some ideas of how to obtain more tight bounds than that in~\eqref{eq:BE} via analyzing the convergence of the series of the Fourier transform of the empirical distribution to the series of the Fourier transform of the normal distibution. Another approach is similar, but substitutes Fourier transform with Laplace transform.

We also plan to verify if the upper bound~\eqref{eq:yup} for the confidence interval of the mean of the rv in \eqref{eq:main} works well for the max norm of the big deviation between the output probability vectors corresponding to unperturbed and attacked images in the test set of CIFAR-10.

% Indeed, one way to estimate the expecatation from above is to use some concentration inequality for a sample mean. For example, one can use Hoeffding’s Inequality:


% \begin{theorem}{(Hoeffding’s Inequality)} 
% Let $\{X_i\}^n_{i=1}$ be independent random variables so
% that $\mathbb{P}(X_i \in [a, b]) = 1$ for some $a < b$, and let $\epsilon > 0.$ Then:

% \begin{itemize}
%     \item $\mathbb{P}(\overline{X_n} - \mathbb{E}[\overline{X_n}] \ge \epsilon) \le e^\frac{-2n\epsilon^2}{(b-a)^2},$
%     \item $\mathbb{P}(|\overline{X_n} - \mathbb{E}[\overline{X_n}]| \ge \epsilon) \le 2e^\frac{-2n\epsilon^2}{(b-a)^2},$
% \end{itemize}

% where $\mathbb{E}[\overline{X_n}] = \sum_{i=1}^n \frac{ \mathbb{E}[X_i]}{n} = \frac{1}{n} \sum_{i=1}^n \mathbb{E}[X_i] = \frac{n \mu}{n} = \mu$ is the population mean (expectation of $X$).
% \end{theorem}

% In the case of random variable $y=\frac{e^{Xt}}{e^{at}},$ and given $\delta = 2e^\frac{-2n\epsilon^2}{(b-a)^2},$ it produces bound for $\epsilon$: $$\epsilon \le \sqrt{\frac{ln(2/ \delta)}{n}} (e^{t-at} - e^{-at})$$ which is exponential w.r.t. $t$, so the probabilistic upper bound for $\mathbb{E}[y]$ looks as $$\mathbb{P}(\mathbb{E}[y] > \overline{X_n} + \epsilon) \le \delta$$ and may be sufficiently overestimated, though decreasing $\sim \frac{C}{\sqrt{\log(n)}}$  with number of samples and still may be used for probabilistic certificates.

% The other thing to consider, is to estimate the stability of empirical bound. 





\subsection{Experiments}
We have conducted experiments aimed at estimating the upper bound of big deviation of output probabilities $\|\vp - \vp^a\|_C$ of the classifiers depending on the way they were trained and on the inference procedure. All experiments are so far conducted on CIFAR-10 with the use of ResNet-18 architecture.
For the estimation of the minimum of Chernoff bounds (w.r.t. parameter $t$) with the use of Bernshtein's idea, we consider $100$ points uniformly distributed on the interval $t \in [10^{-4}, 50]$. For the expectation in equation \eqref{eq:bern}, we use $100$ samples. We compute the max norm for the deviation $\| \vp - \vp^a\|_\infty$.

We present experiments with 2 transforms: rotations and AWGN. In what follows, we use 2 types of model: \texttt{plain} stands for unchanged ResNet-18 training, \texttt{aug} stands for ResNet-18 training with augmentation via random rotations drawn from the von Mises distribution with location and concentration parameters (0,4).
% \texttt{'fmt'} stands for ResNet-18 training with added magnitudes for each color channel in the images. (results are not good)

These models are trained with starting learning rate of $0.1$, using SGD optimizer with momentum of $0.9$. The batch size is $512$. During training, we also augment images with small Gaussian noise with $\sigma=0.01$. The final test accuracies of the models are 93\% and 88\% respectively for \texttt{plain} and \texttt{aug}.

\subsubsection{Rotation transform}
We start with reporting Chernoff bounds for rotation transform. We compute a range of bounds for angles of rotation sampled from intervals $[-\alpha^{\circ},\alpha^{\circ}]$, where $\alpha \in [5,\dots,45]$ with step=5.  Figure~\ref{fig:rotbounds_plain} shows histogram of bounds computed for \texttt{plain} classifier predictions on images in CIFAR-10 test set (10000 images total). As we can see, for smaller angle range of $[-5^{\circ} ,5^{\circ} ]$ (left) the fraction of images with upper bound on the probability of large deviation $\leq 10^{-5}$ is predominating (79.9\%). This fraction monotonically decreases as $\alpha$ grows. With the largest angle range of $[-45^{\circ} ,45^{\circ} ]$ the fraction of such images drops considerably to 22.8\% as with larger angle range it is more likely to have a big deviation in predictions after transformation. \begin{figure}[H]
\centering
\includegraphics[width=0.45\textwidth]{figures/rot_bound5}
\includegraphics[width=0.45\textwidth]{figures/rot_bound45}
\caption{Chernoff bounds on \texttt{plain} classifier predictions deviation $\| \vp - \vp^a \|_C$ after rotation transforms with random angles from $[-5^{\circ} ,5^{\circ} ]$ (left) and $[-45^{\circ} ,45^{\circ} ]$ (right).}
\label{fig:rotbounds_plain}
\end{figure}

We now can take a look at the augmented training model \texttt{aug}.
Figure~\ref{fig:rotbounds_aug} shows a much more moderate drop in the fraction of images with small bound on the big deviations in predictions $\|\vp - \vp^a\|_C$: form 83.2\% for $[-5^{\circ} ,5^{\circ} ]$ (left) to 59.5\% for $[-45^{\circ} ,45^{\circ} ]$ (right). This is in line with the fact that augmented training increases robustness.
\begin{figure}[H]
\centering
\includegraphics[width=0.45\textwidth]{figures/rot_bound5_aug}
\includegraphics[width=0.45\textwidth]{figures/rot_bound45_aug}
\caption{Chernoff bounds on \texttt{aug} classifier predictions deviation $\| \vp - \vp^a \|_C$ after rotation transforms with random angles from $[-5^{\circ} ,5^{\circ} ]$ (left) and $[-45^{\circ} ,45^{\circ} ]$ (right).}
\label{fig:rotbounds_aug}
\end{figure}

\input{figures/rotation}

Figure~\ref{fig:bernrot} shows \emph{robust accuracy}, \emph{certified accuracy} with a fraction of bounds that have values less than $10^{-3}$ (we call it a \emph{small bound}), which we computed using the bound described earlier on CIFAR-10 test set. We denote the fraction of correctly classified images that have small bound ($\leq 10^{-3}$) as \emph{robust accuracy}. We define \emph{certified accuracy} as the fraction of images with small bound that are classified correctly.

Not surprisingly, the fraction of small bounds obtained with \plain{} model (solid {\color{cycle1}blue} line) decreases sharply as we increase the range of angles to sample rotations from. However, \aug{} model (dotted {\color{cycle1}blue} line) shows much more moderate decline. Similar situation is with certified accuracy, where more prone to attacks \plain{} model (solid {\color{cycle6}green} line) falls, while \aug{} model shows less of a decrease (dotted {\color{cycle6}green} line). Robust accuracy ({\color{cycle5}pink} lines) for both models are similar and slightly increase because when bound is smaller, the model is more confident in its prediction and gets more correct classifications.

All in all, we demonstrated that the proposed bound adequately describes the robustness of the models tested with reference to rotation transforms. We now move on to similar analysis on AWGN transform.


%We additionally compute \emph{robust accuracy} - accuracy of predictions with small bounds. We set small bound to be $1e-3$.

\subsubsection{AWGN Transform}
We now take a look on the derived bounds for AWGN attack. We set $\sigma_{max}$ of the transform to the max value stated in the Statement of Work, i.e. $\sigma_{max}=8/255$, and compute the bounds. Figure~\ref{fig:awgnbound} shows that a considerable fraction of images (94\%) have very small bound ($\leq 10^{-5}$) on the deviation after applied AWGN with $\sigma=0.003$, which is roughly 10 times smaller than $\sigma_{max}$. For the $\sigma_{max}$, this fraction drops moderately (to 80\%).
\begin{figure}[H]
\centering
\includegraphics[width=0.49\textwidth]{figures/awgnmin}
\includegraphics[width=0.49\textwidth]{figures/awgnmax}
\caption{Chernoff bounds on \texttt{plain} classifier predictions deviation $\| \vp - \vp^a \|_C$ after AWGN transforms with $\sigma=0.003$ (left) and $\sigma=8/255$ (right).}
\label{fig:awgnbound}
\end{figure}

\input{figures/awgn}

Figure~\ref{fig:bernawgn} shows \emph{robust accuracy}, \emph{certified accuracy} with a fraction of small bounds, computed using the bound described earlier on CIFAR-10 test set for \plain{} model to show robustness metrics with reference to AWGN attack over a range of parameter $\sigma \in [0.003, 8/255]$. The certified accuracy drops from 98.5\% to 83.8\%, while the fraction of small bounds decreases from 97.7\% to 85.5\%. Again, as expected, the robust accuracy grows.


%Note that here are results for two (type of) samples: 
%\begin{itemize}
%    \item $p_1 - p_2 \approx 1.0$, model is very certain in classification;
%    \item $p_1 - p_2 \approx 10^{-2}$, model is very uncertain in classification.
%\end{itemize}
%
%\begin{table}[H]
%\centering
%\caption{Bound estimations: plain training of model} 
%\begin{tabular}{||c c c c||} 
% \hline
% Type of inference & $p_1 - p_2$ & Number of observations of $X$ &  $\min_{t} \frac{\mathbb{E} (e^{Xt})}{e^{at}}$ \\ [0.5ex] 
% \hline\hline
% Plain & 1.00 & 2 & 0.0 \\
%  &  & 5 & 0.0 \\
%  &  & 10 & 0.0 \\
%  &  & 25 & 0.0 \\
%  &  & 100 & 0.0 \\
% & 0.07 & 2 & 1.0006 \\
% &  & 5 & 1.0005 \\
%  &  & 10 & 1.0005 \\
%  &  & 25 & 1.0005 \\
%  &  & 100 & 1.0005 \\ [1ex] 
% \hline
%\end{tabular}
%\label{prob_plain}
%\end{table}
%
%\begin{table}[H]
%\centering
%\caption{Bound estimations: training of model with smoothing} 
%\begin{tabular}{||c c c c||} 
% \hline
% Type of inference & $p_1 - p_2$ & Number of observations of $X$ &  $\min_{t} \frac{\mathbb{E} (e^{Xt})}{e^{at}}$ \\ [0.5ex] 
% \hline\hline
% Plain & 1.00 & 2 & 0.0 \\
%  &  & 5 & 0.0 \\
%  &  & 10 & 0.0 \\
%  &  & 25 & 0.0 \\
%  &  & 100 & 0.0 \\
% & 0.17 & 2 & 1.0006 \\
% &  & 5 & 1.0005 \\
%  &  & 10 & 1.0005 \\
%  &  & 25 & 1.0005 \\
%  &  & 100 & 1.0005 \\ 
%  \hline
% Smoothing & 1.00 & 2 & 0.0 \\
%  &  & 5 & 0.0 \\
%  &  & 10 & 0.0 \\
%  &  & 25 & 0.0 \\
%  &  & 100 & 0.0 \\
% & 0.17 & 2 & 1.0002 \\
% &  & 5 & 1.0002 \\
%  &  & 10 & 1.0002 \\
%  &  & 25 & 1.0002 \\
%  &  & 100 & 1.0002 \\ [1ex] 
% \hline
%\end{tabular}
%\label{prob_smooth}
%\end{table}
%
%
%
%
%
%\begin{table}[H]
%\centering
%\caption{Bound estimations: training of model with double augmentation} 
%\begin{tabular}{||c c c c||} 
% \hline
% Type of inference & $p_1 - p_2$ & Number of observations of $X$ &  $\min_{t} \frac{\mathbb{E} (e^{Xt})}{e^{at}}$ \\ [0.5ex] 
% \hline\hline
% Plain & 1.00 & 2 & 0.0 \\
%  &  & 5 & 0.0 \\
%  &  & 10 & 0.0 \\
%  &  & 25 & 0.0 \\
%  &  & 100 & 0.0 \\
% & 0.007 & 2 & 1.0000 \\
% &  & 5 & 1.0000 \\
%  &  & 10 & 1.0000 \\
%  &  & 25 & 1.0000 \\
%  &  & 100 & 1.0000 \\ 
%  \hline
% Smoothing & 1.00 & 2 & 0.0 \\
%  &  & 5 & 0.0 \\
%  &  & 10 & 0.0 \\
%  &  & 25 & 0.0 \\
%  &  & 100 & 0.0 \\
% & 0.007 & 2 & 1.0000 \\
% &  & 5 & 1.0000 \\
%  &  & 10 & 0.9977 \\
%  &  & 25 & 1.0000 \\
%  &  & 100 & 1.0000 \\ [1ex] 
% \hline
%\end{tabular}
%\label{prob_augaug}
%\end{table}


==> figures/awgn.tex <==
\begin{figure}[ht]
\centering
	\begin{tikzpicture}
	\begin{axis}[
		title=AWGN Transform,
		ylabel={},
		xlabel={$\sigma$},
		xmin=0,
		xmax=0.034,
		ymin=0.8,
		ymax=1,
		legend style={cells={align=left}},
		legend pos = south west,
		width=10cm,
		height=7cm,
	]
	\addlegendimage{ultra thick,color=cycle1};
	\addlegendimage{ultra thick,color=cycle5};
	\addlegendimage{ultra thick,color=cycle6};
		
	\addlegendentry{bound $\leq 10^{-3}$};
	\addlegendentry{robust accuracy};
	\addlegendentry{certified accuracy};

		
	\addplot[thick,color=cycle1,mark=*,mark size=2pt] table[x=sigma,y=frac] {data/awgn|boundfrac.dat};
	
	\addplot[thick,color=cycle5,mark=+,mark size=2pt] table[x=sigma,y=frac] {data/awgn|robacc.dat};
	
	\addplot[thick,color=cycle6,mark=x,mark size=2pt] table[x=sigma,y=frac] {data/awgn|certacc.dat};
		\end{axis}
\end{tikzpicture}
	\caption{Various metrics for \texttt{plain} model over an increasing range of AWGN parameter $\sigma$: ({\color{cycle1}blue}) fraction of bounds $\leq 10^{-3}$, ({\color{cycle5}pink}) robust accuracy, ({\color{cycle6}green}) certified accuracy.}\label{fig:bernawgn}
\end{figure}


==> figures/rotation.tex <==
\begin{figure}[ht]
\centering
	\begin{tikzpicture}
	\begin{axis}[
		title=Rotation Transform,
		ylabel={},
		xlabel={Angles},
		xmin=5,
		xmax=45,
		ymin=0.15,
		ymax=1,
		legend style={cells={align=left}},
		legend pos = south west,
		width=10cm,
		height=7cm,
	]
	\addlegendimage{line legend with two lines={thick, densely dotted, draw=black}{thick,color=black}};
	
%	\addlegendimage{line legend with two lines={thick, densely dotted, draw=cycle2}{ultra thick,color=cycle2}};
	\addlegendimage{ultra thick,color=cycle1};
	\addlegendimage{ultra thick,color=cycle5};
	\addlegendimage{ultra thick,color=cycle6};
	
		\addlegendentry{\texttt{plain}\\ \texttt{aug}};
		
		\addlegendentry{bound $\leq 10^{-3}$};
		\addlegendentry{robust accuracy};
		\addlegendentry{certified accuracy};

		
	\addplot[thick,color=cycle1,mark=*,mark size=2pt] table[x=angle,y=frac] {data/rotation|boundfrac|plain.dat};
	
	\addplot[thick, densely dotted,color=cycle1,mark=*,mark size=2pt] table[x=angle,y=frac] {data/rotation|boundfrac|aug.dat};
	
	
	\addplot[thick,color=cycle5,mark=+,mark size=2pt] table[x=angle,y=frac] {data/rotation|robacc|plain.dat};
	\addplot[thick,densely dotted,color=cycle5,mark=+,mark size=2pt] table[x=angle,y=frac] {data/rotation|robacc|aug.dat};
%	\addlegendentry{\texttt{aug}};
	
	\addplot[thick,color=cycle6,mark=x,mark size=2pt] table[x=angle,y=frac] {data/rotation|certacc|plain.dat};
%	\addlegendentry{\texttt{plain}};
	\addplot[thick,densely dotted,color=cycle6,mark=x,mark size=2pt] table[x=angle,y=frac] {data/rotation|certacc|aug.dat};
%	\addlegendentry{\texttt{aug}};
		\end{axis}
\end{tikzpicture}
	\caption{Various metrics for two models (\texttt{plain} - solid, \texttt{aug} - dotted) over increasing range of angles for sampling of random rotations: ({\color{cycle1}blue}) fraction of bounds $\leq 10^{-3}$, ({\color{cycle5}pink}) robust accuracy, ({\color{cycle6}green}) certified accuracy.}\label{fig:bernrot}
\end{figure}

